VideoXum: Cross-modal Visual and Textural Summarization of Videos

Video summarization aims to distill the most important information from a source video to produce either an abridged clip or a textual narrative. Traditionally, different methods have been proposed depending on whether the output is a video or text, thus ignoring the correlation between the two semantically related tasks of visual summarization and textual summarization. We propose a new joint video and text summarization task. The goal is to generate both a shortened video clip along with the corresponding textual summary from a long video, collectively referred to as a cross-modal summary. The generated shortened video clip and text narratives should be semantically well aligned. To this end, we first build a large-scale human-annotated dataset -- VideoXum (X refers to different modalities). The dataset is reannotated based on ActivityNet. After we filter out the videos that do not meet the length requirements, 14,001 long videos remain in our new dataset. Each video in our reannotated dataset has human-annotated video summaries and the corresponding narrative summaries. We then design a novel end-to-end model -- VTSUM-BILP to address the challenges of our proposed task. Moreover, we propose a new metric called VT-CLIPScore to help evaluate the semantic consistency of cross-modality summary. The proposed model achieves promising performance on this new task and establishes a benchmark for future research.

==> tables/ref_human.tex <==
\begin{table}[t]
\small
\centering
\caption{Selected V2T-SUM Examples.}
\begin{tabularx}{\linewidth}{l|X}
\toprule[1.2pt]
\textbf{Reference} & Two young children are standing in line indoors in what looks like a living room. The little girl is standing closest to the hopscotch mat and she throws her toy onto the mat and then begins jumping until she meets the end of the mat then turns around and heads back to the point she started and her turn is over. The little boy goes next, and he throws the toy onto the mat and begins jumping to the end of the mat, then turns around and jumps back towards his starting point.  The little girl steps in front of the boy and gets into motion to start another turn on the hopscotch mat. \\
\midrule
\textbf{Human}  & Two children stand in front of a mat. They throw something onto the mat. They take turns jumping across the mat. They pick up the item they threw on it. \\
\bottomrule[1.2pt]
\end{tabularx}

\vspace{2mm}
\begin{tabularx}{\linewidth}{l|X}
\toprule[1.2pt]
\textbf{Reference} &  People are in the river in a boat rushing downstream as the water splashes them. A mountain panorama is displayed onscreen. The 6 people row vigorously. We see them from the riverbed looking across, a farm building in the background. A woman talks to the camera. They take group selfies on dry land. People jump from a rock into the river. A man talks to the camera. A man points out the directions to other riders. Another woman talks to the camera. Food is being cooked for the party and plated to the attendees.
 \\ 
\midrule
\textbf{Human}  & A group of rafters are going through turbulent waters. A woman talks to the camera between shots of the rafters. They use their paddles as they go over the falls. \\
\bottomrule[1.2pt]
\end{tabularx}

\label{tab:v2texp}
% \bottomrule
\end{table}

==> tables/tb.tex <==
\begin{table*}[h]
\small
\centering
\caption{In-context learning results on VQAv2, TextVQA, and OK-VQA. 
Both our systems and Flamingo~\cite{alayrac2022flamingo} uses $n=32$ examples in the prompt.
Frozen \cite{tsimpoukelli2021multimodal} uses $n=4$ examples.
The upper part shows the state of the art by supervised/fine-tuned methods.
%\nascomment{maybe label these with how many labeled examples they each use?}\yushi{we used synthesized data from these datasets to train, so maybe it's better not to bring that up}
}
% \begin{tabular}{P{1.7cm}P{1.2cm}P{1.2cm}P{1.0cm}P{1.2cm}P{1.2cm}P{1.2cm}P{1.1cm}P{1.1cm}P{1.1cm}}
\begin{tabular}{lccccccc}
\shline
Method & In-Context & Image & \multicolumn{2}{c}{VQAv2} & \multicolumn{2}{c}{TextVQA} & OK-VQA\\
& Example Retrieval & Representation & test-dev & test-std & val & test & val \\
\shline
\multicolumn{8}{l}{\textbf{Fine-tuned E2E}} \\
%Oscar  &  Feature  & 73.6 & 73.8 \\
%VinVL  & Feature & 75.5 & 75.6 \\
OFA-large \cite{wang2022ofa} & - & Feature  & 80.3 & 80.5 & -& -&-\\
KAT \cite{gui2022kat} & - & Caption + Tags + Feature & - & -& -&- & 54.4\\
GIT \cite{wang2022git} & - & Feature & 78.6 & 78.8 & 59.9 & 59.8 & - \\
%Florence & Feature & 80.2 & 80.4 \\
\shline
\multicolumn{8}{l}{\textbf{In-Context Learning}} \\
Frozen\cite{tsimpoukelli2021multimodal}  & Random & Feature &  38.2 & - & -  & - & 12.6 \\
Flamingo (80B)\cite{alayrac2022flamingo} & Random & Feature & 67.6 & - & 37.9 & - & 57.8 \\
OFA Cap + GPT-3 & Random & Caption & 61.2 & - & 16.5 & -  & 51.2\\
$\ \ $ + Example Selection & CLIP & Caption & 64.9 & - & 22.6 & - & 55.4 \\
PromptCap + GPT-3 & Random & Caption & 72.1 & - & 48.9 & - & 55.3\\
$\ \ $ + Example Selection & CLIP & Caption & \textbf{74.1} & \textbf{74.1} & \textbf{50.9} & \textbf{51.8} & \textbf{
58.8}\\
% GT + GPT-3 & GT-Caption-5 &  59.7 \\
\shline

\end{tabular}
\label{tab:icl}

% \bottomrule
 \vspace{-3mm}
\end{table*}
